Enhancing Human-like Multi-Modal Reasoning: A New Challenging Dataset and Comprehensive Framework

Multimodal reasoning is a critical component in the pursuit of artificial intelligence systems that exhibit human-like intelligence, especially when tackling complex tasks. While the chain-of-thought (CoT) technique has gained considerable attention, the existing ScienceQA dataset, which focuses on multimodal scientific questions and explanations from elementary and high school textbooks, lacks a comprehensive evaluation of diverse approaches. To address this gap, we present COCO Multi-Modal Reasoning(COCO-MMR) dataset, a novel dataset that encompasses an extensive collection of open-ended questions, rationales, and answers derived from the large object dataset COCO. Unlike previous datasets that rely on multiple-choice questions, our dataset pioneers the use of open-ended questions in the context of multimodal CoT, introducing a more challenging problem that effectively assesses the reasoning capability of CoT models. Through comprehensive evaluations and detailed analyses, we provide valuable insights and propose innovative techniques, including multi-hop cross-modal attention and sentence-level contrastive learning, to enhance the image and text encoders. Extensive experiments demonstrate the efficacy of the proposed dataset and techniques, offering novel perspectives for advancing multimodal reasoning. The data and code are available at \href{https://github.com/weijingxuan/COCO-MMR}{https://github.com/weijingxuan/COCO-MMR}.

==> table1.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   \scalebox{0.7}{
%     \begin{tabular}{l|c|cccccccc|c}
%     \toprule
%     Model & Tuned Params & NAT   & SOC   & LAN   & TXT   & IMG   & NO    & G1-6  & G7-12 & AVG \\
%     \midrule
%     Random Choice & -     & 40.28 & 46.13 & 29.25 & 47.45 & 40.08 & 33.66 & 39.35 & 40.67 & 39.83 \\
%     Human  & -     & 90.23 & 84.97 & 87.48 & 89.6  & 87.5  & 88.1  & 91.59 & 82.42 & 88.4 \\
%     \midrule
%     MCAN (Yu et al., 2019) & 95M   & 56.08 & 46.23 & 58.09 & 59.43 & 51.17 & 55.4  & 51.65 & 59.72 & 54.54 \\
%     Top-Down (Anderson et al., 2018) & 70M   & 59.5  & 54.33 & 61.82 & 62.9  & 54.88 & 59.79 & 57.27 & 62.16 & 59.02 \\
%     BAN (Kim et al., 2018) & 112M  & 60.88 & 46.57 & 66.64 & 62.61 & 52.6  & 65.51 & 56.83 & 63.94 & 59.37 \\
%     DFAF (Gao et al., 2019) & 74M   & 64.03 & 48.82 & 63.55 & 65.88 & 54.49 & 64.11 & 57.12 & 67.17 & 60.72 \\
%     ViLT (Kim et al., 2021) & 113M  & 60.48 & 63.89 & 60.27 & 63.2  & 61.38 & 57    & 60.72 & 61.9  & 61.14 \\
%     Patch-TRM (Lu et al., 2021) & 90M   & 65.19 & 46.79 & 65.55 & 66.96 & 55.28 & 64.95 & 58.04 & 67.5  & 61.42 \\
%     VisualBERT (Li et al., 2019) & 111M  & 59.33 & 69.18 & 61.18 & 62.71 & 62.17 & 58.54 & 62.96 & 59.92 & 61.87 \\
%     \midrule
%     UnifiedQABase (Khashabi et al., 2020) & 223M  & 68.16 & 69.18 & 74.91 & 63.78 & 61.38 & 77.84 & 72.98 & 65    & 70.12 \\
%     UnifiedQABase w/ CoT (Lu et al., 2022a) & 223M  & 71    & 76.04 & 78.91 & 66.42 & 66.53 & 81.81 & 77.06 & 68.82 & 74.11 \\
%     \midrule
%     GPT-3.5 (Chen et al., 2020) & 175B  & 74.64 & 69.74 & 76    & 74.44 & 67.28 & 77.42 & 76.8  & 68.89 & 73.97 \\
%     GPT-3.5 w/ CoT (Lu et al., 2022a) & 175B  & 75.44 & 70.87 & 78.09 & 74.68 & 67.43 & 79.93 & 78.23 & 69.68 & 75.17 \\
%     \midrule
%     LLaMA-AdapterT & 1.2M  & 79    & 73.79 & 80.55 & 78.3  & 70.35 & 83.14 & 79.77 & 75.68 & 78.31 \\
%     LLaMA-Adapter & 1.8M  & 84.37 & 88.3  & 84.36 & 83.72 & 80.32 & 86.9  & 85.83 & 84.05 & 85.19 \\
%     Mutimodal-CoTBase & 223M  & 87.52 & 77.17 & 85.82 & 87.88 & 82.9  & 86.83 & 84.65 & 85.37 & 84.91 \\
%     Mutimodal-CoTFlan-T5-large & 783M  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & 93.02 \\
%     \midrule
%     MM-wenge-COTBase  & 229M  & 88.28 & 78.74 & 85.64 & 88.51 & 84.28 & 86.9  & 85.43 & 85.89 & 85.59 \\
%     MM-wenge-COTFlan-T5-large  & 793M  & 97.16 & 84.59 & 93.27 & 96.29 & 90.93 & 94.84 & 93.94 & 92.75 & 93.52 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel}%
% \end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Accuracy on the ScienceQA Dataset. Evaluation across eight categories: Natural Science, Social Science, Linguistics, Textual Context, Image Context, No Context, Grades 1-6, and Grades 7-12. The best results in each category are highlighted in bold.}
  \scalebox{0.7}{
    \begin{tabular}{l|c|cccccccc|c}
    \toprule
    Model                                   & \begin{tabular}[c]{@{}c@{}}Tuned\\ Params\end{tabular} & NAT              & SOC              & LAN              & TXT              & IMG              & NO               & G1-6             & G7-12            & AVG   \\
    \midrule
    Human \cite{DBLP:conf/nips/LuMX0CZTCK22} & -     & 90.23 & 84.97 & 87.48 & 89.6  & 87.5  & 88.10  & 91.59 & 82.42 & 88.40 \\
    \midrule
    MCAN \cite{DBLP:conf/cvpr/Yu0CT019} & 95M   & 56.08 & 46.23 & 58.09 & 59.43 & 51.17 & 55.4  & 51.65 & 59.72 & 54.54 \\
    Top-Down \cite{DBLP:conf/cvpr/00010BT0GZ18} & 70M   & 59.50  & 54.33 & 61.82 & 62.90  & 54.88 & 59.79 & 57.27 & 62.16 & 59.02 \\
    BAN \cite{DBLP:journals/titb/YuPFCS23} & 112M  & 60.88 & 46.57 & 66.64 & 62.61 & 52.6  & 65.51 & 56.83 & 63.94 & 59.37 \\
    DFAF \cite{DBLP:conf/cvpr/GaoJYLHWL19} & 74M   & 64.03 & 48.82 & 63.55 & 65.88 & 54.49 & 64.11 & 57.12 & 67.17 & 60.72 \\
    ViLT \cite{DBLP:conf/icml/KimSK21} & 113M  & 60.48 & 63.89 & 60.27 & 63.2  & 61.38 & 57    & 60.72 & 61.90  & 61.14 \\
    Patch-TRM \cite{lu2021iconqa} & 90M   & 65.19 & 46.79 & 65.55 & 66.96 & 55.28 & 64.95 & 58.04 & 67.50  & 61.42 \\
    VisualBERT \cite{li2019visualbert,DBLP:conf/icml/KimSK21} & 111M  & 59.33 & 69.18 & 61.18 & 62.71 & 62.17 & 58.54 & 62.96 & 59.92 & 61.87 \\
    Mutimodal-CoT$_{\textrm{Base}}$ \cite{DBLP:journals/corr/abs-2302-00923} & 223M  & 87.52 & 77.17 & 85.82 & 87.88 & 82.90  & 86.83 & 84.65 & 85.37 & 84.91 \\
    Mutimodal-CoT$_{\textrm{Flan-T5-large}}$ \cite{DBLP:journals/corr/abs-2302-00923} & 783M  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & 93.02 \\
    \midrule
    UnifiedQA$_{\textrm{Base}}$ \cite{khashabi-etal-2020-unifiedqa} & 223M  & 68.16 & 69.18 & 74.91 & 63.78 & 61.38 & 77.84 & 72.98 & 65.00    & 70.12 \\
    UnifiedQA$_{\textrm{Base}}$ w/ CoT \cite{DBLP:conf/nips/LuMX0CZTCK22} & 223M  & 71    & 76.04 & 78.91 & 66.42 & 66.53 & 81.81 & 77.06 & 68.82 & 74.11 \\
    \midrule
    LLaMA-Adapter$_{\textrm{T}}$ \cite{gao2023llamaadapterv2} & 1.2M  & 79    & 73.79 & 80.55 & 78.30  & 70.35 & 83.14 & 79.77 & 75.68 & 78.31 \\
    LLaMA-Adapter \cite{gao2023llamaadapterv2} & 1.8M  & 84.37 & 88.30  & 84.36 & 83.72 & 80.32 & 86.90  & 85.83 & 84.05 & 85.19 \\
    LLaVa \cite{DBLP:journals/corr/abs-2304-08485} & 13B  & 90.36 & 95.95  & 88.00 & 89.49 & 88.00 & 90.66  & 90.93 & 90.90 & 90.92 \\
    % LLaVa + GPT-4 \cite{DBLP:journals/corr/abs-2304-08485} & 13B  & 91.56 & 96.74  & 91.09 & 90.62 & 88.99 & 93.52  & 92.73 & 92.16 & 92.53 \\
    \midrule
    Enigma-COT$_{\textrm{Base}}$ & 229M  & 88.28 & 78.74 & 85.64 & 88.51 & 84.28 & 86.90  & 85.43 & 85.89 & 85.59 \\
    Enigma-COT$_{\textrm{Flan-T5-large}}$ & 793M  & \textbf{97.51} &  \textbf{84.70} &  \textbf{94.73} &  \textbf{96.68} &  \textbf{91.37} &  \textbf{95.89} &  \textbf{94.46} &  \textbf{93.47} & \textbf{94.11} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel1}%
\end{table*}%




==> table3.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   \scalebox{0.7}{
%     \begin{tabular}{lrrrrrrrrrr}
%     \toprule
%     Model & \multicolumn{1}{l}{NAT} & \multicolumn{1}{l}{SOC} & \multicolumn{1}{l}{LAN} & \multicolumn{1}{l}{TXT} & \multicolumn{1}{l}{IMG} & \multicolumn{1}{l}{NO} & \multicolumn{1}{l}{G1-6} & \multicolumn{1}{l}{G7-12} & \multicolumn{1}{l}{AVG} & \multicolumn{1}{l}{rouge} \\
%     \midrule
%     Mutimodal-CoT Base & 13.72 & 15.3  & 13.27 & 13.59 & 14.43 & 13.66 & 14.35 & 13.18 & 13.94 & 96.97 \\
%     Enigma-COT\$\_{Base}\$   w/ Multi-hop  w/ Back CL & 22.38 & 18.9  & 20.09 & 21.21 & 21.07 & 21.18 & 21.62 & 20.04 & 21.06 & 96.99 \\
%     Enigma-COT\$\_{Flan-T5 large }\$  w/ Multi-hop  w/ Back CL & 22.38 & 18.9  & 20.09 & 21.21 & 21.07 & 21.18 & 21.62 & 20.04 & 21.06 & 98.37 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel3}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Investigation into the Improvement of Rational Generation by Enigma-COT Model, where the first stage of the generation paradigm is replaced with Enigma-COT. RougeL is used as the evaluation metric. 'w/' indicates the inclusion of a particular module.'w/' indicates the inclusion of a particular module.}
%   \scalebox{0.7} {
%     \begin{tabular}{l|c}
%     \toprule
%   Model                                             & \multicolumn{1}{r}{ RougeL} \\
%     \midrule
%     Mutimodal-CoT$_{Base}$ &96.97 \\
%     Enigma-COT$_{Base}$ &96.99 \\
%     Enigma-COT$_{Flan-T5-large}$ &98.37 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel3}%
% \end{table}%



==> table4.tex <==

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   \scalebox{0.7}{
%     \begin{tabular}{lrrrrrrrrr}
%     \toprule
%     Model & \multicolumn{1}{l}{NAT} & \multicolumn{1}{l}{SOC} & \multicolumn{1}{l}{LAN} & \multicolumn{1}{l}{TXT} & \multicolumn{1}{l}{IMG} & \multicolumn{1}{l}{NO} & \multicolumn{1}{l}{G1-6} & \multicolumn{1}{l}{G7-12} & \multicolumn{1}{l}{AVG} \\
%     \midrule
%     Mutimodal-CoT Base & 87.52 & 77.17 & 85.82 & 87.88 & 82.9  & 86.83 & 84.65 & 85.37 & 84.91 \\
%     Enigma-COT\$\_{Base}\$   w/ Multi-hop  w/ Back CL & 88.28 & 78.74 & 85.64 & 88.51 & 84.28 & 86.9  & 85.43 & 85.89 & 85.59 \\
%     Enigma-COT\$\_{Flan-T5 large }\$  w/ Multi-hop  w/ Back CL & 97.16 & 84.59 & 93.27 & 96.29 & 90.93 & 94.84 & 93.94 & 92.75 & 93.52 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel4}%
% \end{table*}%


% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Results Obtained by Re-training the Second Stage with Enigma-COT Based on the Rational Generation from Base or Flan-T5 Large in the First Stage as shown in Table 3. 'w/' indicates the inclusion of a particular module.}
%   \scalebox{0.7} {
%     \begin{tabular}{l|rrrrrrrrr}
%     \toprule
%     Model & \multicolumn{1}{l}{NAT} & \multicolumn{1}{l}{SOC} & \multicolumn{1}{l}{LAN} & \multicolumn{1}{l}{TXT} & \multicolumn{1}{l}{IMG} & \multicolumn{1}{l}{NO} & \multicolumn{1}{l}{G1-6} & \multicolumn{1}{l}{G7-12} & \multicolumn{1}{l}{AVG} \\
%     \midrule
%     Mutimodal-CoT$_{Base}$ & 87.52 & 77.17 & 85.82 & 87.88 & 82.9  & 86.83 & 84.65 & 85.37 & 84.91 \\
%     Enigma-COT$_{Base w/ Multi-hop; Back CL}$ & 88.28 & 78.74 & 85.64 & 88.51 & 84.28 & 86.9  & 85.43 & 85.89 & 85.59 \\
%     Enigma-COT$_{Flan-T5 large w/ Multi-hop; Back CL}$ & 97.16 & 84.59 & 93.27 & 96.29 & 90.93 & 94.84 & 93.94 & 92.75 & 93.52 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel4}%
% \end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Results Obtained by Re-training the Second Stage with Enigma-COT Based on the Rational Generation from Base or Flan-T5 Large in the First Stage as shown in Table 3. 'w/' indicates the inclusion of a particular module.}
%   \scalebox{0.7} {
%     \begin{tabular}{l|r}
%     \toprule
%     Model & \multicolumn{1}{l}{AVG} \\
%     \midrule
%     Mutimodal-CoT$_{Base}$  & 84.91 \\
%     Enigma-COT$_{Base}$ & 85.59 \\
%     Enigma-COT$_{Flan-T5-large}$ & 93.52 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel4}%
% \end{table}%


==> table5.tex <==
%     % Table generated by Excel2LaTeX from sheet 'Sheet1'
%     \begin{table}[htbp]
%       \centering
%       \caption{Performance Comparison of Various Models on the COCO-MMR Dataset.}
%       \scalebox{0.45}{
%       \begin{tabular}{llllll}
%         \toprule
%         \textbf{Model}                                                                                      & \textbf{type}                                                    & \textbf{\begin{tabular}[c]{@{}l@{}}Tuned\\ Params\end{tabular}} & \textbf{BLUE}  &  \textbf{Similarity} & \textbf{Rouge} \\ 
%         \midrule
%         Human                                                                                               & Human                                                            & -------                                                         & 80.35          & 90.25                                      & 82.73                                 \\ 
%         \midrule
%      \begin{tabular}[c]{@{}l@{}}Mutimodal-CoT\\ $_{Flan-T5-Large}$ \cite{DBLP:journals/corr/abs-2302-00923}\end{tabular} & \begin{tabular}[c]{@{}l@{}}VQA\\ Mutimodal model\end{tabular}    & 783M                                                            &  66.89          &        79.77                       &        69.04                        \\ 
%         \midrule
%          UnifiedQA$_{Base}$ \cite{khashabi-etal-2020-unifiedqa}    & Text-to-text  & 223M                                                            & 43.76          & 63.97                                      & 39.46                                 \\
%         UnifiedQA$_{Base}$ w/ COT \cite{DBLP:conf/nips/LuMX0CZTCK22}                                                                 & Text-to-text                                                        & 223M                                                  & 64.71 & 75.75                             & 66.62                        \\ 

%         \midrule
%         LLAVA \cite{DBLP:journals/corr/abs-2304-08485}            & \begin{tabular}[c]{@{}l@{}}Mutimodal \\ LLM model\end{tabular}   & 13B                                                             & 59.38          & 74.59                                      & 62.15                                 \\ 
%         \midrule
%         Enigma-COT$_{Base}$                                                                 & Ours                                                             & 229M                                                            & 65.52          & 78.03                                      & 67.67                                 \\
%         Enigma-COT$_{Flan-T5-large}$                                                                  & Ours                                                             & 793M                                                            & \textbf{68.07} & \textbf{80.41}                             & \textbf{70.17}                        \\ 
%         \bottomrule
%         \end{tabular}
%     }
%   \label{tab:addlabel5}%
% \end{table}%

\begin{table}[htbp]
\small
\centering
\caption{Performance Comparison of Various Models on the COCO-MMR Dataset.}
{\renewcommand\baselinestretch{1.2}\selectfont
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
Model & Type & Tuned Params & BLUE & Similarity & Rouge \\ 
\midrule
Human & Human & - & 80.35 & 90.25 & 82.73 \\ 
\hline
Mutimodal-CoT$_{\textrm{Flan-T5-Large}}$ & VQA & 783M &  66.89 & 79.77 & 69.04 \\ 
\hline
UnifiedQA$_{\textrm{Base}}$& Text-to-text  & 223M & 43.76 & 63.97 & 39.46 \\
UnifiedQA$_{\textrm{Base}}$ w/ COT & Text-to-text & 223M & 64.71 & 75.75 & 66.62 \\ 
\hline
LLAVA           & LLM & 13B & 59.38 & 74.59 & 62.15 \\ 
\hline
Enigma-COT$_{\textrm{Base}}$ & Ours & 229M & 65.52 & 78.03 & 67.67 \\
Enigma-COT$_{\textrm{Flan-T5-large}}$ & Ours & 793M & \textbf{68.07} & \textbf{80.41} & \textbf{70.17} \\ 
\bottomrule
\end{tabular}\par}
}
\label{tab:addlabel5}
\end{table}

==> table6.tex <==
    % Table generated by Excel2LaTeX from sheet 'Sheet1'
%     \begin{table}[htbp]
%       \centering
%       \caption{Performance Comparison of Various Models on the COCO-MMR Dataset. This table presents the performance comparison among different model categories including human, Text-to-text LM, VQA Multimodal, Multimodal LLM, and our proposed COT-COT model performance on the COCO-MMR dataset.}
%       \scalebox{0.7}{
%       \begin{tabular}{llll}
%         \hline
%         \textbf{Model}                 & \textbf{\begin{tabular}[c]{@{}l@{}}Tuned\\ Params\end{tabular}} & \textbf{similarity} & \textbf{rouge} \hline
%         Enigma-COT$_{unifiedqa\_base}$       & 229M                                                            & 85.56                                      & 61.25                                 \\
%         Enigma-COT$_{unifiedqa\_large}$      & 748M                                                            & 86.49                                      & 62.83                                 \\
%         Enigma-COT$_{Flan-T5 base}$ & 253M                                                   & 86.62                             & 62.91                        \\
%         Enigma-COT$_{Flan-T5 large}$         & 793M                                                            & 87.23                                      & 64.25                                 \\ \hline
%         \end{tabular}
%     }
%   \label{tab:addlabel6}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%     \centering
%     \caption{Performance metrics of Enigma-COT's first stage (rationale generation) on the COCO-MMR Dataset, with a particular focus on Rouge scores.}
%     \scalebox{0.6}{
%     \begin{tabular}{lllll}
%       \toprule
%       \textbf{Model}                 & \textbf{\begin{tabular}[c]{@{}l@{}}Tuned\\ Params\end{tabular}} & \textbf{BLUE} & \textbf{Similarity} & \textbf{Rouge}  \\ 
%       \midrule
%       Enigma-COT$_{\textrm{unifiedqa\_base}}$       & 229M                                                          &67.41  & 85.56                                      & 61.25                                 \\
%       Enigma-COT$_{\textrm{unifiedqa\_large}}$      & 748M &68.62 & 86.49                                  & 62.83                                 \\
%       Enigma-COT$_{\textrm{Flan-T5 base}}$ & 253M                                            &68.74           & 86.62                             & 62.91                        \\
%       Enigma-COT$_{\textrm{Flan-T5 large}}$         & 793M                                   &69.90                         & 87.23                                      & 64.25                                 \\ 
%       \bottomrule
%       \end{tabular}
%   }
%   \label{tab:addlabel6}%
%   \end{table}%
  
  
      % Table generated by Excel2LaTeX from sheet 'Sheet1'
    \begin{table}[htbp]
        \centering
        \caption{Performance metrics of Enigma-COT's first stage (rationale generation) on the COCO-MMR Dataset, with a particular focus on Rouge scores.}
        {\renewcommand\baselinestretch{1.2}\selectfont
  \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccc}
          \toprule
          Model  & Tuned Params & BLUE  &  Similarity & Rouge \\ 
          \midrule
          
          Enigma-COT$_{\textrm{unifiedqa\_base}}$       & 229M                                                          &67.41  & 85.56                                      & 61.25                                 \\
      Enigma-COT$_{\textrm{unifiedqa\_large}}$      & 748M &68.62 & 86.49                                  & 62.83                                 \\
      Enigma-COT$_{\textrm{Flan-T5 base}}$ & 253M                                            &68.74           & 86.62                             & 62.91                        \\
      Enigma-COT$_{\textrm{Flan-T5 large}}$         & 793M                                   &69.90                         & 87.23                                      & 64.25                                 \\ 
      \bottomrule
          \end{tabular}
      }\par}
    \label{tab:addlabel6}%
  \end{table}%
  
  
  
 
